not-so-BigGAN: Generating High-Fidelity Images on Small Compute with Wavelet-based Super-Resolution

State-of-the-art models for high-resolution image generation, such as BigGAN and VQVAE-2, require an incredible amount of compute resources and/or time (512 TPU-v3 cores) to train, putting them out of reach for the larger research community. On the other hand, GAN-based image super-resolution models, such as ESRGAN, can not only upscale images to high dimensions, but also are efficient to train. In this paper, we present not-so-big-GAN (nsb-GAN), a simple yet cost-effective two-step training framework for deep generative models (DGMs) of high-dimensional natural images. First, we generate images in low-frequency bands by training a sampler in the wavelet domain. Then, we super-resolve these images from the wavelet domain back to the pixel-space with our novel wavelet super-resolution decoder network. Wavelet-based down-sampling method preserves more structural information than pixel-based methods, leading to significantly better generative quality of the low-resolution sampler (e.g., 64x64). Since the sampler and decoder can be trained in parallel and operate on much lower dimensional spaces than end-to-end models, the training cost is substantially reduced. On ImageNet 512x512, our model achieves a Fr\'echet Inception Distance (FID) of 10.59 -- beating the baseline BigGAN model -- at half the compute (256 TPU-v3 cores).

==> figs/fid_is.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.75,0.75}
\definecolor{color1}{rgb}{0.886274509803922,0.290196078431373,0.2}
\definecolor{color2}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color3}{rgb}{0.596078431372549,0.556862745098039,0.835294117647059}
\definecolor{color4}{rgb}{0.75,0,0.75}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
legend cell align={left},
legend columns=8,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1.1,-0.1)}, anchor=north, draw=white!80!black, fill=white!89.8039215686275!black},
tick align=outside,
tick pos=left,
title={(a) Truncation levels: [1.0, 0.4, 0.1, 0.01]},
x grid style={white},
xlabel={Inception Score (IS)},
xmajorgrids,
xmin=21.7744506835937, xmax=353.872399902344,
xtick style={color=white!33.3333333333333!black},
y dir=reverse,
y grid style={white},
ylabel={Fréchet Inception Distance (FID)},
ymajorgrids,
ymin=0, ymax=80,
ytick style={color=white!33.3333333333333!black}
]
\addplot [semithick, color0]
table {%
36.8698120117188 46.1262758692844
90.151123046875 36.7254714423349
114.954147338867 45.2638167606489
113.785743713379 59.0998729639798
};
\addlegendentry{not-so-BigGAN}
\addplot [semithick, color1]
table {%
67.8924255371094 48.1742808707574
68.8363571166992 46.8467803627878
72.8854064941406 58.1257476924467
71.0080795288086 77.1785817027479
};
\addlegendentry{not-so-BigGAN-pixel}
\addplot [semithick, color2]
table {%
124.703018188477 23.5220091016631
211.611373901367 28.1503892989335
217.339935302734 36.7551872655889
214.112869262695 47.8340419854819
};
\addlegendentry{BigGAN $+$ not-so-BigGAN decoder}
\addplot [semithick, color3]
table {%
111.004898071289 23.244376705362
203.309036254883 25.7143266494527
215.922760009766 33.457463617481
209.613327026367 43.9201331755549
};
\addlegendentry{BigGAN $+$ not-so-BigGAN-pixel decoder}
\addplot [semithick, white!46.6666666666667!black]
table {%
213.248336791992 10.655149511664
326.865661621094 21.0446221289729
338.777038574219 29.028895283939
329.445861816406 39.2289976788491
};
\addlegendentry{BigGAN}
\addplot [semithick, red, mark=*, mark size=3, mark options={solid}, only marks]
table {%
218.352630615234 2.6041947196598
};
\addlegendentry{Validation set - Reconstructions}
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}, only marks]
table {%
132.588592529297 13.7897916477402
};
\addlegendentry{Validation set - Original}
\addplot [semithick, color4, mark=*, mark size=3, mark options={solid}, only marks]
table {%
96.4408111572266 20.3710414377554
};
\addlegendentry{not-so-BigGAN FID$^*$}

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={(b) Truncation levels: [1.0, 0.8, 0.6, 0.5, 0.4, 0.2, 0.1, 0.01]},
x grid style={white},
xlabel={Inception Score (IS)},
xmajorgrids,
xmin=32.8829204559326, xmax=120.594534683228,
xtick style={color=white!33.3333333333333!black},
y dir=reverse,
y grid style={white},
ylabel={Fréchet Inception Distance (FID)},
ymajorgrids,
ymin=0, ymax=80,
ytick style={color=white!33.3333333333333!black}
]
\addplot [semithick, color0]
table {%
36.8698120117188 46.1262758692844
58.9217720031738 38.6979778030176
84.675178527832 35.600417543587
96.1155090332031 35.7342399205941
90.151123046875 36.7254714423349
116.607643127441 41.0855308511218
114.954147338867 45.2638167606489
113.785743713379 59.0998729639798
};
\end{groupplot}

\end{tikzpicture}

